LoViT: Long Video Transformer for Surgical Phase Recognition

Online surgical phase recognition plays a significant role towards building contextual tools that could quantify performance and oversee the execution of surgical workflows. Current approaches are limited since they train spatial feature extractors using frame-level supervision that could lead to incorrect predictions due to similar frames appearing at different phases, and poorly fuse local and global features due to computational constraints which can affect the analysis of long videos commonly encountered in surgical interventions. In this paper, we present a two-stage method, called Long Video Transformer (LoViT) for fusing short- and long-term temporal information that combines a temporally-rich spatial feature extractor and a multi-scale temporal aggregator consisting of two cascaded L-Trans modules based on self-attention, followed by a G-Informer module based on ProbSparse self-attention for processing global temporal information. The multi-scale temporal head then combines local and global features and classifies surgical phases using phase transition-aware supervision. Our approach outperforms state-of-the-art methods on the Cholec80 and AutoLaparo datasets consistently. Compared to Trans-SVNet, LoViT achieves a 2.4 pp (percentage point) improvement in video-level accuracy on Cholec80 and a 3.1 pp improvement on AutoLaparo. Moreover, it achieves a 5.3 pp improvement in phase-level Jaccard on AutoLaparo and a 1.55 pp improvement on Cholec80. Our results demonstrate the effectiveness of our approach in achieving state-of-the-art performance of surgical phase recognition on two datasets of different surgical procedures and temporal sequencing characteristics whilst introducing mechanisms that cope with long videos.

==> 2-RelatedWork.tex <==

\section{Related Work}

Statistical models were the core techniques behind early work for surgical phase recognition.
%{Earliest attempts for surgical phase recognition mainly adopted statistical models.}
Blum~\etal~\cite{DBLP:conf/miccai/BlumFN10} analyzed surgery signals and tool usage for dimensionality reduction of video frames into image features.
Padoy~\etal~\cite{DBLP:journals/mia/PadoyBAFBN12} processed synchronized signals based on Dynamic Time Warping~\cite{Dynamic_1978} and Hidden Markov Models(HMM)~\cite{DBLP:journals/pieee/Rabiner89}.  Bardram~\etal~\cite{DBLP:conf/percom/BardramDJLNP11} presented a sensor platform and a machine learning approach to sense surgical phases. Holden~\etal~\cite{DBLP:journals/tbe/HoldenUSMCGPF14} developed a workflow segmentation algorithm for needle interventions using needle tracking data. 
However, these techniques operate on extra information, such as manual annotation or equipment installation, that might be inconvenient to collect and could cause workload, rather than only video. 
Pure video-based methods were then proposed to overcome the aforementioned limitations.
Quellec~\etal~\cite{DBLP:journals/tmi/QuellecLCC15} presented a multiscale motion characterization approach based on adaptive spatiotemporal polynomials.% \added[id=AG]{for ...}. 
~Dergachyova~\etal~\cite{DBLP:journals/cars/DergachyovaBHMJ16} trained a set of \textit{AdaBoost} classifiers capable of distinguishing one surgical phase from others, and then adopted a Hidden semi-Markov Model to obtain a final decision. 
Since vision features and temporal context of surgical video are highly complex, these methods show limited representation capacities with pre-defined dependencies~\cite{DBLP:journals/tmi/JinD0YQFH18,DBLP:conf/miccai/GaoJLDH21}.
\input{Images/LoViT_main}

With the advent of deep learning, completely new methodology was proposed for pure video inputs.
EndoNet~\cite{DBLP:journals/tmi/TwinandaSMMMP17} is the first work to use a Convolutional Neural Network (CNN) for multiple recognition tasks, extracted spatial features and designed a hierarchical HMM for modeling temporal information.
Twinanda~\cite{DBLP:phd/hal/Twinanda17} used Long Short-term Memory (LSTM), a type of Recurrent Neural Network (RNN) gate, rather than an HMM to enhance EndoNet's ability to understand the temporal context.
Jin~\etal~\cite{DBLP:journals/mia/JinLDCQFH20} presented a multi-task framework called MTRCNet-CL, which used a correlation loss to exploit the relatedness between tool presence detection and surgical phase recognition with the aim of simultaneously boosting the performance of both tasks. 
Similar to early work, these methods need extra annotation, increasing workload and cost. 
Moreover, some datasets don't contain such annotation, so these methods are unsuitable for all datasets. As a result, some approaches focused on learning a single task only.
SV-RCNet~\cite{DBLP:journals/tmi/JinD0YQFH18} leveraged a Residual network (ResNet)~\cite{resnet_he} and an LSTM network to end-to-end learn spatial and temporal features, respectively. 
Yi~\etal~\cite{DBLP:conf/miccai/YiJ19} presented an Online Hard Frame Mapper (OHFM) to handle the detected hard frames with indistinguishable visual features but separately assigned with different labels. Gao~\etal~\cite{DBLP:conf/icra/GaoJDH20} designed a framework using a tree search algorithm to consider future information from LSTM. 
However, LSTMs are only able to retain memory spanning limited sequence lengths. This particularly affects their use on surgical videos for temporal feature extraction since interventions could last a few hours~\cite{DBLP:conf/miccai/CzempielPKSFKN20}. 
To address this problem, Czempiel~\etal~\cite{DBLP:conf/miccai/CzempielPKSFKN20} presented TeCNO, based on Temporal Convolutional Networks (TCNs)~\cite{DBLP:conf/eccv/LeaVRH16, DBLP:conf/cvpr/FarhaG19}, that is able to extract long-term temporal information. 
However, by essentially adapting dilated convolutions~\cite{DBLP:conf/ssw/OordDZSVGKSK16} for long sequences using TCNs, temporal information, particularly that of fine-grained relationships can be lost. 

With the rise of Transformers in Natural Language Processing (NLP)~\cite{DBLP:conf/nips/VaswaniSPUJGKP17}, the parallel nature of attention blocks were quickly used to replace CNNs and RNNs architectures. In vision-related tasks, Vision Transformer (ViT)~\cite{DBLP:conf/iclr/DosovitskiyB0WZ21} was proposed by replacing word tokens of vanilla Transformers with sequences of 16-by-16 pixels image patches.
Temporal attention was then introduced with TimeSformer~\cite{gberta_2021_ICML} and VideoViT~\cite{DBLP:conf/iccv/Arnab0H0LS21} approaches for video classification with self-attention on sequences of frame-level patches. 
The Anticipative Video Transformer (AVT)~\cite{DBLP:conf/iccv/GirdharG21} then ranked first in EPIC-Kitchens-100 Challenge~\cite{Damen2022RESCALING} by using a ViT backbone and a causal head layer to predict the next actions with the disadvantage of working only on dozens of frames long videos.
Czempiel~\etal~\cite{DBLP:conf/miccai/CzempielPOKBN21} first introduced a transformer-based temporal future extractor for surgical phase recognition. This was followed up by Trans-SVNet~\cite{DBLP:conf/miccai/GaoJLDH21}, that despite tailing a small Transformer model to search for the possible loss of temporal information by fusing temporal features from the TCN with previous spatial features, fine-grained relationships are still lost. This problem exacerbates since time and memory complexity of Transformers are quadratic due to their dot-product operations, a particular problem for long videos commonly resulting from surgical interventions.
%}{However, Tansformer requires the quadratic times dot-product and memory usage.}
% you already talked about this problem with LSTMs above
%\deleted[id=AG]{Similar problem with LSTM, it also can't span long duration, which is fatal in surgical video.}

%With the rise of Transformers in NLP~\cite{ref_AttnIsAllYouNeed}, the parallel nature of attention blocks were quickly used to replace RNNs' sequential architecture. Czempiel et al. first introduced a transformer-based method for online surgical phase recognition. Their method, OperA~\cite{ref_OperA}, use a CNN for visual feature extraction followed by multiple self-attention layers. Trans-SVNet~\cite{ref_TransSVNet} reconsidered the combined effect of spatial and temporal features by reusing the spatial embedding after extracting the temporal features from the TCN, and fusing both embeddings into a transformer layer for surgical phase recognition. Although those approaches reach a high accuracy, they fail to capture longer term relations between video frames sampled at a high frame rate.

%In recent years, Transformers architectures emerged and are still evolving at a fast pace. First used in NLP, they quickly were adopted to vision with the initial Vision Transformer (ViT)~\cite{ref_ViT} replacing word tokens with instead a sequence of 16-by-16 pixels image patches. Later, the Swin Transformer~\cite{ref_Swin} translated CNNs' inductive biases to the ViT by incorporating hierarchical increase of image patches size. Like convnets, this leads to larger receptive fields as the model becomes deeper. Also, shifting windows allows for cross-window connection and limiting self-attention computation with non-overlapping local windows. Transformers require more data compared to their CNNs counter part as they have less structured inductive bias and therefore need to learn more from the data representation. This led vision transformers to become the new state-of-the-art in object detection, segmentation, classification on multiple datasets~\cite{ref_DeiT}. Temporal attention was then suggested by the TimeSformer~\cite{ref_TimeSformer} and VideoViT~\cite{ref_ViViT} for video classification with self-attention on sequences of frames-level patches, but could only to over one minute long videos. As mentioned, long surgical videos have strong local redundancy and complex global dependency between video frames. UniFormer~\cite{ref_Uniformer} seamlessly addresses this problem by integrating merits of 3D convnets and spatiotemporal self-attention blocks. Surgical anticipation in the OR plays a key role for improving patients outcomes. The Anticipative Video Transformer (AVT)~\cite{ref_AVT} ranked first in EPIC-Kitchens-100 Challenge, uses a ViT backbone and causal head layer to predict next actions.

%Other transformer-based models brings the original self-attention operation, which scales quadratically with the sequence length with pairwise interactions, to a L.Log.L~\cite{ref_Reformer} or linear relation~\cite{ref_LongFormer, ref_Linformer}.

To address the limitations of Transformers on long sequence inputs, Informer~\cite{DBLP:conf/aaai/ZhouZPZLXZ21} uses attention to capture precise long-range dependency in videos. For this, it tackles three inherent problems of Transformers, namely their quadratic time complexity and high memory usage of $\mathcal{O}(L^2)$, as well as the inherent limitations of the encoder-decoder architecture by introducing a novel \textit{ProbSparse} self-attention mechanism, which achieves $\mathcal{O}(L \log L)$ time complexity and ("and" make it not very clear what are the 3 problems) memory usage.

%While today's video recognition systems can process snapshots or short clips accurately, they are unable to learn spatial and temporal representations across longer time spans. State-of-the-art architectures \added[id=AG]{typically process videos at 1~Hz and} can only process less than 5 seconds of a video without hitting the computation and memory bottlenecks of computing infrastructure. Long videos with high frame rate (HFR) are computationally expensive as they require more time to process and memory on hardware. This causes an increase in processing time and memory requirements. Hence, performing surgical phase recognition during long surgeries\added[id=AG]{, whilst keeping fine-grained temporal information,} can quickly become difficult to perform at scale.

%To overcome these limitations, 
Inspired by these works, our method relies on a Transformer-based~\cite{DBLP:conf/nips/VaswaniSPUJGKP17} framework. 
To achieve accurate surgical phase recognition, our model needs to rely on more effective spatial feature extraction mechanisms. 
For this purpose, we adopt video clip-level supervision to decrease the ambiguity of similar frames appearing at different surgical phases. Moreover, for our model to process long videos with less information lost, we adopt a multi-scale temporal aggregation and fusion module consisting of self-attention and \textit{ProbSparse} self-attention that extract short and long temporal features, respectively. 
Last, we use heatmap-guided supervision to better model phase transitions. 
Through extensive experiments, we find evidence to support that our strategies have an improvement in the performance of surgical phase recognition on two publicly available datasets.
%With the second  train a rich feature extractor,   we introduce \textit{LoViT}, a Long Video Transformer for Surgical Phase Recognition.
%With this new approach, our aim is 1) to increase the number of frames per second for more fine-grained phase transitions and to speed up online feedback in the operating room, 2) to achieve state of the art on phase recognition with long temporal range in videos, and 3) \replaced[id=AG]{to guarantee}{keep} a constant inference time with increasing video length.
%\textit{Contributions} 
%Through extensive experiments, we demonstrate that our framework generalizes to different laparoscopic video datasets, i.e. Cholec80 and m2cai16 and compete with state-of-the-art architectures, e.g. AVT, and Trans-SVNet.
%Our contributions are summarized as follows:
%\begin{itemize}
%    \item \deleted[id=AG]{We propose }a transformer-based method to recall and attend all frames in long videos.
%    \item \replaced[id=AG]{a leverage of}{We leverage} the full temporal resolution from surgical videos for phase recognition.
%    \item \replaced[id=AG]{an evaluation}{We evaluate LoViT} on two popular surgical video datasets.
%    \item \deleted[id=AG]{We achieve }a constant inference speed with increasing video length.
%\end{itemize}

==> Images/Fig_Fuse_Trans.tex <==
\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{Images/Fuse_Trans_cut.pdf}
\caption{The architecture of our multi-scale temporal fusion module MF-Tans. The MF-Trans embodies a 2-layer vanilla self-attention block~(grey dotted box) and a 1-layer vanilla self-attention block to receive two-branch inputs~(grey line and black line), respectively.}
\label{fig:fusetrans}
\centering
\end{figure}

==> Images/Fig_Global_Trans.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{Images/Global_Trans_v4_cut.pdf}
\caption{The architecture of our global temporal module framework G-Informer. The G-Informer module embodies $m_g$-layer \textit{ProbSparse} self-attention~(grey dotted box) and $n_g$-layer vanilla self-attention~(black dotted box) blocks to receive two-branch inputs~(grey line and black line), respectively.}
\label{fig:globaltrans}
\centering
\end{figure}

==> Images/Fig_visualize_autolaparo.tex <==

\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{Images/Visualization_sota_autolaparo_crop.pdf}
\caption{Qualitative comparisons with some other methods on AutoLaparo dataset. Two videos, Video 15 and Video 16, are presented in the first and second columns, respectively, in the AutoLaparo dataset. The top three rows show the phase prediction results obtained by AVT and LoViT, as well as their corresponding Ground Truth $\mathrm{GT}_p$, with different colors denoting different phases. The last two rows display the heatmap prediction output by our proposed LoViT, denoted as $\hat{h}$, and its corresponding Ground Truth $\mathrm{GT}_h$}
\label{fig:visualize_comparewithsotaautolaparo}
\centering
\end{figure*}

==> Images/Fig_visualize_spatial_tsne.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{Images/TSNE_visulize_crop_2.pdf}
\caption{Visualization for the spatial feature distribution of different extractors using the t-SNE method. Point set: Video frames of Video 60 in Cholec80. Different Colors: different tool annotations. First row: the spatial feature distribution of the frame-only spatial feature extractor in Trans-SVNet. Second row: the spatial feature distribution of the temporally-rich spatial feature extractor in our LoViT. Different columns present different perplexity parameters in t-SNE.}
\label{fig:visual_spatial_tsne}
\centering
\end{figure*}

==> Tables/Ablationstudy_Data_augmentation.tex <==

\begin{table}[]

%\renewcommand\arraystretch{1.2}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\toprule[1pt]    
Dataset &$\mathcal{D}$ & $\mathrm{Accuracy}$ & $\mathrm{Precision}$ & $\mathrm{Recall}$ & $\mathrm{Jaccard}$\\\hline

%\multicolumn{2}{c|}{VI} & \multirow{2}{*}{Time (s)} \\ \cline{3-12}
%                                      && ODS         & OIS        & ODS        & OIS        & ODS        & OIS        & ODS         & OIS        & ODS         & OIS &\\\midrule[1pt]
\multirow{2}{*}{Cholec80} &           & ?      & ?       & ?        & ?\\ \cline{2-6}
&\checkmark           & ?      & ?       & ?        & ?\\ \hline

%\bottomrule[1pt] 
\multirow{2}{*}{AutoLaparo} &           & ?      & ?       & ?        & ?\\ \cline{2-6}
&\checkmark           & $\bf{79.53 \pm 8.36}$      & \bf{79.61}       & \bf{64.85}        & \bf{53.74}\\ \hline

%\bottomrule[1pt] 
\end{tabular}}
\end{center}

\caption{Effects of Data Augmentation ($\mathcal{D}$) on Cholec80
and AutoLaparo datasets.}
\label{tab:dataaugmentation}
\end{table}

==> egbib.tex <==
\begin{thebibliography}{00}
% TODO Make sure all references are formatted similarly


% Surgical Data Science - Artificial Intelligence

\bibitem{ref_SDS}
Le  na Maier-Heina, Matthias Eisenmann, ..., Nicolas Padoy, Pierre Jannin, and Stefanie Speidel.
Surgical Data Science – from Concepts to Clinical Translation, (2020)

\bibitem{ref_cai4cai}
Tom Vercauteren, Mathias Unberath, Nicolas Padoy, Nassir Navab
CAI4CAI: The Rise of Contextual Artificial Intelligence in Computer-Assisted Interventions. (2020)

% Surgical phase, workflow recognition papers

\bibitem{ref_SPR_sysrev}
Garrow, C.R., Kowalewski, K-F., Li, L., Wagner, M., Schmidt, M.W., Engelhardt, S., Hashimoto, D.A., Kenngott, H.G., Bodenstedt, S., Speidel, S., Müller-Stich, B.P., Nickel, F.: Machine Learning for Surgical Phase Recognition. In Annals of Surgery \textbf{273}(4), 684-693 (2021)

\bibitem{ref_LSTM}
S. Hochreiter, J. Schmidhuber: Long Short-Term Memory. In: 
Transactions on Medical Imaging \textbf{36}(1), 1718-1724 (1997)

\bibitem{ref_HMM_Padoy}
N. Padoy, T. Blum, H. Feussner, M-O. Berger, N. Navab: On-line Recognition of Surgical Activity for Monitoring in the Operating Room. In: AAAI
Transactions on Medical Imaging \textbf{36}(1), 1718-1724 (2008)

\bibitem{ref_m2cai16}
Twinanda, A.P., Mutter, D., Marescaux, J., de Mathelin, M., Padoy, N.: Singleand multi-task architectures for surgical workflow challenge at M2CAI 2016. arXiv
preprint arXiv:1610.08844 (2016)

\bibitem{ref_EndoNet}
Twinanda, A.P., Shehata, S., Mutter, D., Marescaux, J., De Mathelin, M., Padoy, N.: Endonet: a deep architecture for recognition tasks on laparoscopic videos. In: IEEE
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2017)

\bibitem{ref_EndoLSTM}
Twinanda, A.P.: Vision-based approaches for surgical activity recognition using laparoscopic and RBGD videos. Ph.D. thesis, Strasbourg (2017)

\bibitem{ref_MTRCNet-CL}
Y. Jin, H. Li, Q. Dou, H. Chen, J. Qin, C. Fu, P. Heng.: Multi-Task Recurrent Convolutional Network with Correlation Loss for Surgical Video Analysis. (2019)

\bibitem{ref_3DCNN}
I. Funke, S. T. Mees, J. Weitz, S. Speidel.: Video-based surgical skill assessment using 3D convolutional neural networks. IJCARS 14.7 (2019) pp. 1217-1225 (2019)

\bibitem{ref_InstructionGen}
Jinglu, Z.: Surgical Instruction Generation with Transformers. In: MICCAI 2021
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2021)

\bibitem{ref_WorkflowAnticip}
Kun, Y.: Surgical workflow anticipation using instrument interaction. In: MICCAI 2021
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2021)

\bibitem{ref_TCN}
C. Lea, R. Vidal, A. Reiter, G. D. Hager.: Temporal Convolutional Networks: A Unified Approach to Action Segmentation. In: ECCV
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2016)

\bibitem{ref_TeCNO}
Czempiel, T., Paschali, M., Matthias Keicher, Walter Simson, Hubertus Feussner, Seong Tae Kim, Nassir Navab.: TeCNO: Surgical Phase Recognition with Multi-Stage Temporal Convolutional Networks. In: MICCAI 2020
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2020)

\bibitem{ref_OperA}
Czempiel, T., Paschali, M., Matthias Keicher, Walter Simson, Hubertus Feussner, Seong Tae Kim, Nassir Navab.: OperA: Attention-Regularized Transformers for Surgical Phase Recognition. In: MICCAI 2021
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2021)

\bibitem{ref_WorkflowAnticip}
Kun, Y.: Surgical workflow anticipation using instrument interaction. In: MICCAI 2021
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2017)

\bibitem{ref_TransSVNet}
Xiaojie, G., Yueming, J., Yonghao, L., Qi, D., and Pheng-Ann, H..: Trans-SVNet: Accurate Phase Recognition from Surgical Videos via Hybrid Embedding Aggregation Transformer. In: MICCAI 2021
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2017)

\bibitem{ref_MTMS-TCN}
Twinanda, A.P..: Multi-Task Temporal Convolutional Networks for Joint Recognitionof  Surgical  Phases  and Steps  in  Gastric  Bypass  Procedure. In: IEEE
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2021)



% Transformers and Attentions models
\bibitem{ref_AttnIsAllYouNeed}
Ashish Vaswani, Noam Shazeer, Niki Parmar, Jakob Uszkoreit, Llion Jones, Aidan N. Gomez, Lukasz Kaiser, Illia Polosukhin.: Attention Is All You Need. In: 
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2021)

\bibitem{ref_Uniformer}
Kunchang Li, Yali Wang, Peng Gao, Guanglu Song, Yu Liu, Hongsheng Li, Yu Qiao.: UniFormer: Unified Transformer for Efficient Spatiotemporal Representation Learning. In: 
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2021)

\bibitem{ref_Swin}
Ze Liu, Yutong Lin, Yue Cao, Han Hu, Yixuan Wei, Zheng Zhang, Stephen Lin, Baining Guo.: Swin Transformer: Hierarchical Vision Transformer using Shifted Windows. In: 
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2021)

\bibitem{ref_AVT}
Rohit Girdhar, Kristen Grauman.: Anticipative Video Transformer. In: 
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2021)

\bibitem{ref_TimeSformer}
Gedas Bertasius, Heng Wang, Lorenzo Torresani.: Is  Space-Time  Attention  All  You  Need  for  Video  Understanding?. In: 
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2021)

\bibitem{ref_ViViT}

\bibitem{ref_ViT}
Alexey Dosovitskiy, Lucas Beyer, Alexander Kolesnikov, Dirk Weissenborn, Xiaohua Zhai, Thomas Unterthiner, Mostafa Dehghani, Matthias Minderer, Georg Heigold, Sylvain Gelly, Jakob Uszkoreit, Neil Houlsby.: An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale. In: 
Transactions on Medical Imaging \textbf{36}(1), 86–97 (2021)

% Pytorch frameworks, github repos, cv datasets

\bibitem{ref_timm}
Ross Wightman.:PyTorch Image Models, 2019, GitHub, GitHub repository, 10.5281/zenodo.4414861, https://github.com/rwightman/pytorch-image-models

\bibitem{ref_ImageNet}
He, K., Zhang, X., Ren, S., Sun, J.: Deep residual learning for image recognition. In:
Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition.
pp. 770–778 (2016) 2, 4, 6

\bibitem{conf/ipcai/KaticWGKMDS14}
Darko Katic, Anna{-}Laura Wekerle, R{\"{u}}diger Dillmann, and Stefanie Speidel, ``Knowledge-Driven Formalization of Laparoscopic Surgeries for Rule-Based Intraoperative Context-Aware Assistance,'' Information Processing in Computer-Assisted Interventions - 5th International Conference, {IPCAI} 2014, Fukuoka, Japan, June 28, 2014.
% High frame rate papers

% Long video papers
\bibitem{ref_Informer}
Haoyi Zhou, Shanghang Zhang, Jieqi Peng, Shuai Zhang, Jianxin Li, Hui Xiong, Wancai Zhang.: Informer: Beyond Efficient Transformer for Long Sequence Time-Series Forecasting

\bibitem{ref_BeyondShortClips}
Xitong Yang, Haoqi Fan, Lorenzo Torresani, Larry Davis, Heng Wang.: Beyond Short Clips: End-to-End Video-Level Learning with Collaborative Memories.






\bibitem{ref_article1}
Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

\bibitem{ref_lncs1}
Author, F., Author, S.: Title of a proceedings paper. In: Editor, F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
Springer, Heidelberg (2016). \doi{10.10007/1234567890}

\bibitem{ref_book1}
Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
Location (1999)

\bibitem{ref_proc1}
Author, A.-B.: Contribution title. In: 9th International Proceedings
on Proceedings, pp. 1--2. Publisher, Location (2010)

\bibitem{ref_url1}
LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
Oct 2017

\bibitem{journals/cars/BlumPFN08}
Tobias Blum, Nicolas Padoy, Hubertus Feußner, and Nassir Navab, ``
Workflow mining for visualization and analysis of surgeries,'' Int. J. Comput. Assist. Radiol. Surg. 3(5): 379-386 (2008)

\bibitem{journals/jbi/BouarfaJD11}
Loubna Bouarfa, Pieter P. Jonker, and Jenny Dankelman, ``Discovery of high-level tasks in the operating room,'' J. Biomed. Informatics 44(3): 455-462 (2011)

\bibitem{conf/miccai/AhmadiSSHFN06}
Seyed-Ahmad Ahmadi, Tobias Sielhorst, Ralf Stauder, Martin Horn, Hubertus Feußner, Nassir Navab:
Recovery of Surgical Workflow Without Explicit Models. MICCAI (1) 2006: 420-428

\bibitem{conf/mmvr/ReileyLVVKYH08}
	Carol E. Reiley, Henry C. Lin, Balakrishnan Varadarajan, Bal{\'{a}}zs V{\'{a}}gv{\"{o}}lgyi, Sanjeev Khudanpur, David D. Yuh, and Gregory D. Hager, ``
Automatic Recognition of Surgical Motions Using Statistical Modeling for Capturing Variability,'' MMVR 2008: 396-401

\bibitem{conf/miccai/BlumFN10}
Tobias Blum, Hubertus Feußner, Nassir Navab:
Modeling and Segmentation of Surgical Workflow from Laparoscopic Video. MICCAI (3) 2010: 400-407

\bibitem{journals/mia/ZappellaHHV13}
Luca Zappella, Benjamín Béjar Haro, Gregory D. Hager, René Vidal:
Surgical gesture classification from video and kinematic data. Medical Image Anal. 17(7): 732-745 (2013)

\bibitem{journals/tbe/LalysRBJ12}
Florent Lalys, Laurent Riffaud, David Bouget, Pierre Jannin:
A Framework for the Recognition of High-Level Surgical Tasks From Video Images for Cataract Surgeries. IEEE Trans. Biomed. Eng. 59(4): 966-976 (2012)

\bibitem{DBLP:journals/tmi/QuellecLCC15}
Gw{\'{e}}nol{\'{e}} Quellec, Mathieu Lamard, B{\'{e}}atrice Cochener, and Guy Cazuguel:
Real-Time Task Recognition in Cataract Surgery Videos Using Adaptive Spatiotemporal Polynomials. IEEE Trans. Medical Imaging 34(4): 877-887 (2015)

\bibitem{DBLP:journals/cars/DergachyovaBHMJ16}
	Olga Dergachyova, David Bouget, Arnaud Huaulmé, Xavier Morandi, Pierre Jannin:
Automatic data-driven real-time segmentation and recognition of surgical workflow. Int. J. Comput. Assist. Radiol. Surg. 11(6): 1081-1089 (2016)

\end{thebibliography}
